Modeling Musical Structure with Artificial Neural Networks

In recent years, artificial neural networks (ANNs) have become a universal tool for tackling real-world problems. ANNs have also shown great success in music-related tasks including music summarization and classification, similarity estimation, computer-aided or autonomous composition, and automatic music analysis. As structure is a fundamental characteristic of Western music, it plays a role in all these tasks. Some structural aspects are particularly challenging to learn with current ANN architectures. This is especially true for mid- and high-level self-similarity, tonal and rhythmic relationships. In this thesis, I explore the application of ANNs to different aspects of musical structure modeling, identify some challenges involved and propose strategies to address them. First, using probability estimations of a Restricted Boltzmann Machine (RBM), a probabilistic bottom-up approach to melody segmentation is studied. Then, a top-down method for imposing a high-level structural template in music generation is presented, which combines Gibbs sampling using a convolutional RBM with gradient-descent optimization on the intermediate solutions. Furthermore, I motivate the relevance of musical transformations in structure modeling and show how a connectionist model, the Gated Autoencoder (GAE), can be employed to learn transformations between musical fragments. For learning transformations in sequences, I propose a special predictive training of the GAE, which yields a representation of polyphonic music as a sequence of intervals. Furthermore, the applicability of these interval representations to a top-down discovery of repeated musical sections is shown. Finally, a recurrent variant of the GAE is proposed, and its efficacy in music prediction and modeling of low-level repetition structure is demonstrated.

==> Chapters/seg1/seg1.tex <==



\chapter{Probabilistic Segmentation of Musical Sequences using Restricted Boltzmann Machines}

% keep this commented out for blind review:
\newcommand\Mark[1]{\textsuperscript#1}

%\author{Stefan Lattner\Mark{1}, Maarten Grachten\Mark{1}, Kat Agres\Mark{2}, Carlos E. Cancino Chac\'{o}n\Mark{1}}
%\institute{\Mark{1} Austrian Research Institute for Artificial Intelligence\\\Mark{2} Queen Mary, University of London}

\begin{abstract}
A salient characteristic of human perception of music is that musical events are perceived as being grouped temporally into structural units such as phrases or motifs.
Segmentation of musical sequences into structural units is a topic of ongoing research, both in cognitive psychology and music information retrieval.
Computational models of music segmentation are typically based either on explicit knowledge of music theory or human perception, or on statistical and information-theoretic properties of musical data.
The former, rule-based approach has been found to better account for (human annotated) segment boundaries in music than probabilistic approaches~\cite{Pearce:2010ij}, although the statistical model proposed in~\cite{Pearce:2010ij} performs almost as well as state-of-the-art rule-based approaches.
In this paper, we propose a new probabilistic segmentation method, based on Restricted Boltzmann Machines (RBM).
By sampling, we determine a probability distribution over a subset of visible units in the model, conditioned on a configuration of the remaining visible units.
We apply this approach to an n-gram representation of melodies, where the RBM generates the conditional probability of a note given its n-1 predecessors.
We use this quantity in combination with a threshold to determine the location of segment boundaries.
A comparative evaluation shows that this model slightly improves segmentation performance over the model proposed in~\cite{Pearce:2010ij}, and as such is closer to the state-of-the-art rule-based models.
\end{abstract}

\section{Introduction}\label{sec:Introduction}

Across perceptual domains, grouping and segmentation mechanisms are crucial for our disambiguation and interpretation of the world.
Both top-down, schematic processing mechanisms and bottom-up, grouping mechanisms contribute to our ability to break the world down into meaningful, coherent ``chunks''.
Indeed, a salient characteristic of human perception of music is that musical sequences are not experienced as an indiscriminate stream of events, but rather as a sequence of temporally contiguous musical groups or segments.
Elements within a group are perceived to have a coherence that leads to the perception of these events as a structural unit (e.g., a musical phrase or motif).

The origin and nature of this sense of musical coherence, or lack thereof, which gives rise to musical grouping and segmentation has been a topic of ongoing research.
A prominent approach from music theory and cognitive psychology has been to apply perceptual grouping mechanisms, such as those suggested by Gestalt psychology, to music perception.
\emph{Gestalt principles}, such as the laws of proximity, similarity, and closure, were first discussed in visual perception \cite{wertheimer1938laws}, and have been successfully applied to auditory scene analysis \cite{bregman90} and inspired theories of music perception \cite{meyer56,narmour90,lerdahl1983generative}.
Narmour’s Implication-Realization theory \cite{narmour90}, for example, uses measures of pitch proximity and closure that offer insight into how listeners perceive the boundaries between musical phrases.
This type of theory-driven approach has given rise to various rule-based computational models of segmentation.
This class of models relies upon the specification of one or more principles according to which musical sequences are grouped.

A second class of computational methods is based on statistical and information theoretic properties of musical data.
Recent research in this area has used the statistical structure of sequential tonal and temporal information to compute measures of information (such as Information Content), which serve as a proxy for expectedness (see for example, \cite{agresinformation}).
Measures of expectation may then be used to calculate segmentation boundaries.
For example, a highly expected musical event followed by an unexpected event is often indicative of a perceptual boundary.

A comparison of rule-based and probabilistic approaches~\cite{Pearce:2010ij} suggests the most effective segmentation methods are generally theory-based approaches.
The statistical model proposed in~\cite{Pearce:2010ij} (IDyOM) is capable of much better segmentations than simpler statistical models based on digram transition probabilities and point-wise mutual information~\cite{Brent99anefficient}, but still falls slightly short of state-of-the-art rule-based models.
Even if rule-based models currently outperform statistical models, there is a motivation to further pursue statistical models of melodic segmentation.

It is plausible that the rules put forth in music-theoretic and perception-based models have been induced by regularities in musical and auditory stimuli. Models that learn directly from the statistics of such stimuli are conceptually simpler than models that describe the perceptual mechanisms of human beings that have internalized the regularities of those stimuli.

In this paper, we introduce a new probabilistic segmentation method, based on a class of stochastic neural networks known as Restricted Boltzmann Machines (RBMs). 
We present a Monte-Carlo method to determine a probability distribution over a subset of visible units in the model, conditioned on a configuration of the remaining visible units.
Processing melodies as n-grams, the RBM generates the conditional probability of a note given its n-1 predecessors.
This quantity, in combination with a threshold, determines the location of segment boundaries.
In Section~\ref{sec:Related} we give a brief overview of both rule-based and statistical models for melodic segmentation, where we restrict ourselves to an overview of the models with which we compare our approach: those evaluated in ~\cite{Pearce:2010ij}.
Then, we will argue that our model (explained in Section~\ref{sec:Method}) has advantages over statistical models based on n-gram counting. In addition to this qualitative comparison of our method to other approaches (Section~\ref{sec:Method}), we reproduce a quantitative evaluation experiment by Pearce et al.~\cite{Pearce:2010ij} (Section~\ref{sec:Experiment}). The results, as reported and discussed in Section~\ref{sec:results}, show that our model slightly improves segmentation performance over IDyOM, and as such is closer to the state-of-the-art rule-based models. Finally, we present conclusions and directions for future work in Section~\ref{sec:Conclusion and Future Work}.

\section{Related Work}\label{sec:Related}

\subsection{Rule based segmentation}\label{sec:rule-based-segm}

One of the first models of melodic segmentation based on Gestalt rules was proposed by Tenney and Polansky in~\cite{Tenney:1980wf}.
This theory quantifies rules of local detail to predict grouping judgements.
However, this theory does not account for vague or ambiguous grouping judgements, and the selection of their numerical weights is rather arbitrary \cite{Tenney:1980wf,lerdahl1983generative}.
 One of the most popular music theoretic approaches is Lerdahl and Jackendoff's Generative Theory of Tonal Music (GTTM) \cite{lerdahl1983generative}.
This theory pursues the formal description of musical intuitions of experienced listeners   through a combination of cognitive principles and generative linguistic theory.
In GTTM,
the hierarchical segmentation of a musical piece into motifs, phrases and sections is represented through a \emph{grouping structure}.
This structure is expressed through consecutively numbered \emph{grouping preference rules} (GPRs), which model possible structural descriptions that correspond to experienced listeners' hearing of a particular piece \cite{lerdahl1983generative}.
According to GTTM, two types of evidence are involved in the determination of the grouping structure.
The first kind of evidence to perceive a phrase boundary between two melodic events is \emph{local detail}, i.e.\ relative temporal proximity like slurs and rests  (GPR 2a), inter-onset-interval (IOI) (GPR 2b) and change in register (GPR 3a), dynamics (GPR 3b), articulation (GPR 3c) or duration (GPR 3d).

The organization of \emph{larger-level} grouping involves intensification of the effects picked out by GPRs 2 and 3 on a larger temporal scale (GPR 4), symmetry (GPR 5) and parallelism (GPR 6).
While Lerdahl and Jackendoff's work did not attempt to quantify these rules, a computational model for identification of segment boundaries that numerically quantifies the GPRs 2a, 2b, 3a and 3d was proposed by Frankland and Cohen \cite{Frankland:2004ug}.
This model encodes melodic profiles using absolute duration of the notes, and MIDI note numbers for representing absolute pitch.

A related model to the quantification of the GPRs was proposed by Cambouropoulos \cite{Cambouropoulos:2001vj}.
The Local Boundary Detection Model (LBDM) consists of a \emph{change} rule and a \emph{proximity} rule, operated over melodic profiles that encode pitch, IOI and rests.
On the one hand, the change rule identifies the strength of a segment boundary in relation to the degree of change between consecutive intervals  (similar to GPR 3).
On the other hand, the proximity rule considers the size of the intervals involved (as in GPR 2).
The total boundary strength is then computed as a weighted sum of the boundaries for pitch, IOI and rests, where the weights were empirically selected.

Temperley \cite{Temperley:2001wm} introduced a similar method, called Grouper, that partitions a melody (represented by onset time, off time, chromatic pitch and a level in a metrical hierarchy) into non-overlapping groups.
 Grouper uses three \emph{phase structure preference rules} (PSPR) to asses the existence of segment boundaries.
PSPR 1 locates boundaries at large IOIs and large offset-to-onset intervals (OOIs), and is similar to GPR 2, while PSPR 3 is a rule for metrical parallelism, analogous to GPR 6.
PSPR 2 relates to the length of the phrase, and was empirically determined by Temperley using the Essen Folk Song Collection (EFSC), and therefore, may not be a general rule~\cite{pearce2010role}.


\subsection{Statistical and information theoretic segmentation}\label{sec:stat-inform-theor}

In \cite{pearce2010role}, Pearce, M\"ullensiefen and Wiggins applied two information theoretic approaches, originally designed by Brent~\cite{Brent99anefficient} for  word identification in unsegmented speech, to construct boundary strength profiles (BSPs) for melodic events. This method relies on the assumption that segmentation boundaries are located in places where certain information theoretic measures have a higher numerical value than in the immediately neighbouring locations. The first approach constructs BSPs using transition probability (TP),  the conditional probability of an element of a sequence given the preceding element, while the second method relies on pointwise mutual information (PMI), that measures to which degree the occurrence of an event reduces the model's uncertainty about the co-occurrence of another event, to produce such BSPs

Inspired by developments in musicology, computational linguistics and machine learning, Pearce, M\"ullensiefen and Wiggins offered the IDyOM model.
IDyOM is an unsupervised, multi-layer, variable-order Markov model that computes the conditional probability and Information Content (IC) of a musical event, given the prior context.
An overview of IDyOM can be found in~\cite{Pearce:2010ij}.

\section{Method}\label{sec:Method}

The primary assumption underlying statistical models of melodic segmentation is that the perception of segment boundaries is induced by the statistical properties of the data. RBMs (Section~\ref{sec:rbm}) can be trained effectively as a generative probabilistic model of data (Section~\ref{sec:Training}), and are therefore a good basis for defining a segmentation method. However, in contrast to sequential models such as recurrent neural networks, RBMs are models of static data, and do not model temporal dependencies. A common way to deal with this is to feed the model sub-sequences of consecutive events (n-grams) as if they were static entities, without explicitly encoding time. This n-gram approach allows the model to capture regularities among events that take place within an n-gram. With some simplification we can state that these regularities take the form of a joint probability distribution over all events in an n-gram. With Monte-Carlo methods, we can use this joint distribution to approximate the conditional probability of some of these events, given others. This procedure is explained in Sections~\ref{sec:appr-prob-v} and~\ref{sec:Posterior}.

\newcommand{\idy}{IDyOM}

\subsection{Relation to other statistical models}\label{sec:relation-idyom-model}
Although our RBM-based method works with n-gram representations just as the statistical methods discussed in Section~\ref{sec:stat-inform-theor}, the approaches are fundamentally different.
Models such as \idy{}, TP and PMI are based on n-gram counting, and as such has to deal with the trade-off between longer n-grams and sparsity of data that is inevitable when working with longer sub-sequences.
In \idy{}, this problem is countered with ``back-off'' a heuristic to dynamically decrease or increase the n-gram size as the sparsity of the data allows.
In contrast, an RBM does not assign probabilities to n-grams based directly on their frequency counts.
The non-linear connections between visible units (via a layer of hidden units) allow a much smoother probability distribution, that can also assign non-zero probability to n-grams that were never presented as training data.
As a result, it is possible to work with a fixed, relatively large n-gram size, without the need to reduce the size in order to counter data sparsity.

Every computational model requires a set of basic features that describe musical events.
In \idy{}, these basic features are treated as statistically independent, and dependencies between features are modelled explicitly by defining combined viewpoints as cross-products of subsets of features.
An advantage of the RBM model is that dependencies between features are modelled as an integral part of learning, without the need to specify subsets of features explicitly.

Finally, the statistical methods discussed in Section~\ref{sec:Related} are fundamentally n-gram based, and it is not obvious how these methods can be adapted to work with polyphonic music rather than monophonic melodies.
Although the RBM model presented here uses an n-gram representation, it is straight-forward to adopt the same segmentation approach using a different representation of musical events, such as the note-centred representation proposed in~\cite{grachten14:_asses_learn_score_featur_model}.
This would make the RBM suitable for segmenting polyphonic music.

\subsection{Restricted Boltzmann Machines} \label{sec:rbm}
An RBM is a stochastic Neural Network with two layers, a visible layer with units $\mathbf{v} \in \{0,1\}^r$ and a hidden layer with units $\mathbf{h} \in \{0,1\}^q$ \cite{Hinton:2002ic}.
The units of both layers are fully interconnected with weights $\mathbf{W} \in \mathbb{R}^{r \times q}$, while there are no connections between the units within a layer.

In a trained RBM, the marginal probability distribution of a visible configuration $\mathbf{v}$ is given by the equation
\begin{equation}
p(\mathbf{v}) = \frac{1}{Z} \sum_{\mathbf{h}}{e^{-E(\mathbf{v}, \mathbf{h})}},
\end{equation}
where $E(\mathbf{v}, \mathbf{h})$ is an energy function.
The computation of this probability distribution is usually intractable, because it requires summing over all possible joint configurations of $\mathbf{v}$ and $\mathbf{h}$ as
\begin{equation}
Z = \sum_{\mathbf{v},\mathbf{h}}{e^{-E(\mathbf{v},\mathbf{h})}}.
\end{equation}

\subsection{Approximation of the probability of $v$ }\label{sec:appr-prob-v}

Another way to compute the probability of a visible unit configuration $\mathbf{v}$ is to approximate it through Monte Carlo techniques.
To that end, for $N$ randomly initialized \emph{fantasy particles}\footnote{See \cite{tielemanPcd2008}} $\mathbf{Q}$, we execute Gibbs sampling until thermal equilibrium. 
In the visible \emph{activation vector} $\mathbf{q}_i$ of a fantasy particle $i$, element $q_{ij}$ specifies the probability that visible unit $j$ is on.
Since all visible units are independent given $\mathbf{h}$, the probability of $\mathbf{v}$ based on one fantasy particle's visible activation is computed as:

\begin{equation}
p(\mathbf{v} | \mathbf{q}_i) = \prod_j{p(v_j | q_{ij})}.
\end{equation}

As we are using binary units, such an estimate can be calculated by using a binomial distribution with one trial per unit.
We average the results over $N$ fantasy particles, leading to an increasingly close approximation of the true probability of $\mathbf{v}$ as N increases:

\begin{equation}\label{binomial}
p(\mathbf{v} | \mathbf{Q}) = \frac{1}{N}\sum_i^N{\prod_j{\binom{1}{v_j}q_{ij}^{v_j}(1-q_{ij})^{1-v_j}}}.
\end{equation}

\subsection{Posterior probabilities of visible units}\label{sec:Posterior}
When the visible layer consists of many units, $N$ will need to be very large to obtain good probability estimates with the method described above.
However, for conditioning a (relatively small) subset of visible units $\mathbf{v}_y \subset \mathbf{v}$ on the remaining visible units $\mathbf{v}_x = \mathbf{v} \setminus \mathbf{v}_y$, the above method is very useful.
This can be done by Gibbs sampling after randomly initializing the units $\mathbf{v}_y$ while clamping all other units $\mathbf{v}_x$ according to their initial state in $\mathbf{v}$.
In Eq.
\ref{binomial}, all $\mathbf{v}_x$ contribute a probability of $1$, which results in the conditional probability of $\mathbf{v}_y$ given $\mathbf{v}_x$.

We use this approach to condition the units belonging to the last time step of an n-gram on the units belonging to preceding time steps. For the experiments reported in this paper, we found that it is sufficient to use 150 fantasy particles and for each to perform 150 Gibbs sampling steps.

\subsection{Training}\label{sec:Training}

We train a single RBM using \emph{persistent contrastive divergence} (PCD)~\cite{tielemanPcd2008} with \emph{fast weights}~\cite{tielemanFpcd2009}, a variation of the standard \emph{contrastive divergence} (CD) algorithm~\cite{hinton06}.
PCD is more suitable for sampling than CD, because it results in a better approximation of the likelihood gradient.

Based on properties of neural coding, sparsity and selectivity can be used as constraints for the optimization of the training algorithm~\cite{Goh:2010wi}.
Sparsity encourages competition between hidden units, and selectivity prevents over-dominance by any individual unit.
A parameter $\mu$ specifies the desired degree of sparsity and selectivity, whereas another parameter $\phi$ determines how strongly the sparsity/selectivity constraints are enforced. 

\subsection{Data Representation}\label{sec:DataRepresentation}

From the monophonic melodies, we construct a set of n-grams by using a sliding window of size n and a step size of 1.
For each note in the n-gram, four basic features are computed: 1) absolute values of the pitch interval between the note and its predecessor (in semitones); 2) the contour (up, down, or equal); 3) inter-onset-interval (IOI); and 4) onset-to-offset-interval (OOI). The IOI and OOI values are quantized into semiquaver and quaver, respectively.
Each of these four features is represented as a binary vector and its respective value for any note is encoded in a one-hot representation. The first n-1 n-grams in a melody are noise-padded to account for the first n-1 prefixes of the melody. Some examples of binary representations of n-grams are given in Figure~\ref{fig:Representation}).

\begin{figure}[t]
\centering\footnotesize
\includegraphics[width=0.8\linewidth]{Chapters/seg1/fig/ngrams.pdf}
\caption{Seven examples of n-gram training instances (n=10) used as input to the RBM.
Within each instance (delimited by a dark gray border), each of the 10 columns represents a note.
Each column consists of four \emph{one-hot} encoded viewpoints: $|$\emph{interval}$|$, \emph{contour}, \emph{IOI} and \emph{OOI} (indicated by the braces on the left). The viewpoints are separated by horizontal light gray lines for clarity.
The first instance shows an example of noise padding (in the first six columns) to indicate the beginning of a melody.}
\label{fig:Representation}
\end{figure}

\subsection{Information Content}

\begin{figure}[t]
\centering\footnotesize
\includegraphics[width=1.\linewidth]{Chapters/seg1/fig/bs_curve.pdf}
\caption{A BSP calculated from 11-grams.
The upper figure shows the notes of 9 measures (36 beats) of a German folk song.
The lower figure shows a BSP (i.e. IC) used for segmentation.
The correct segmentation (ground truth) is depicted as vertical grey bars at the top of the figures, segment boundaries found by our model are shown as dashed vertical lines.
Note that the BSP has particularly high peaks at rests and at high intervals.
However, the segment boundary found at beat $28$ does not have any of those cues and was still correctly classified.}
\label{fig:bs_curve}
\end{figure}

After training the model as described in \ref{sec:Training}, we estimate the probability of the last note conditioned on its preceding notes for each n-gram as introduced in \ref{sec:Posterior}.
From the probabilities $p(e_t \mid e_{t-n+1}^{t-1})$ computed thus, we calculate the IC as:

\begin{equation}
h(e_t \mid e_{t-n+1}^{t-1}) = log_2 \frac{1}{p(e_t \mid e_{t-n+1}^{t-1})},
\end{equation}
where $e_t$ is a note event at time step t, and $e_k^l$ is a note sequence from position $k$ to $l$ of a melody.
IC is a measure of the unexpectedness of an event given its context.
According to a hypothesis of~\cite{Pearce:2010ij}, segmentation in auditory perception is determined by perceptual expectations for auditory events.
In this sense, the IC relates directly to this perceived boundary strength, thus we call the IC over a note sequence \emph{boundary strength profile}.

\subsection{Peak Picking}
Based on the BSP described in the previous section, we need to find a concrete binary segmentation vector.
For that, we use the peak picking method described in~\cite{Pearce:2010ij}.
This method finds all peaks in the profile and keeps those which are $k$ times the standard deviation greater than the mean boundary strength, linearly weighted from the beginning of the melody to the preceding value:

\begin{equation}
S_n > k \sqrt{\frac{\sum_{i=1}^{n-1}{(w_i S_i - \bar{S}_{w,1\dots n-1})^2}}{\sum_1^{n-1}{w_i}}} + \frac{\sum_{i=1}^{n-1}{w_i S_i}}{\sum_1^{n-1}{w_i}},
\end{equation}
where $S_m$ is the $m$-th value of the BSP, and $w_i$ are the weights which emphasize recent values over those of the beginning of the song (triangular window), and $k$ has to be found empirically.

\section{Experiment}\label{sec:Experiment}

\subsection{Training Data}\label{sec:TrainingData}

In this work, we use the EFSC \cite{TheEssenFolksongC:1995um}.
This database is a widely used corpus in MIR for experiments on symbolic music.
This collection consists of more than 6000 transcriptions of folk songs primarily from Germany and other European regions.
The EFSC collection is commonly used for testing computational models of music segmentation, due to the fact that it is annotated with phrase markers.

In accordance with~\cite{Pearce:2010ij}, we used the \emph{Erk} subset of the EFSC, which consists of 1705 German folk melodies with a total of $78,995$ note events.
Phrase boundary annotations are marked at about $12\%$ of the note events.

\subsection{Procedure}
The model is trained and tested on the data described in Section~\ref{sec:TrainingData}, with n-gram lengths varying between 1 and 11. For each n-gram length, we perform 5-fold cross-validation and average the results over all folds.
Similar to the approach in~\cite{Pearce:2010ij}, after computing the BSPs, we evaluate different $k$ from the set $\{0.70, 0.75, 0.80, 0.85, 0.90, 0.95, 1.00\}$ and choose the value that maximizes F1 for the respective n-gram length.
To make results comparable to those reported in~\cite{Pearce:2010ij}, the output of the model is appended with an implicit (and correct) phrase boundary at the end of each melody.

Since the hyper-parameters of the model are inter-dependent, it is infeasible to exhaustively search for the optimal parameter setting.
For the current experiment, we have manually chosen a set of hyper-parameters that give reasonable results for the different models tested: 200 hidden units, a batch size of 100, a momentum of 0.6, and a learning rate of 0.007 which we linearly decrease to zero during training.
The fast weights used in the training algorithm (see Section~\ref{sec:Training}) help the fantasy particles mix well, even with small learning rates.
The learning rate of the fast weights is increased from 0.002 to 0.007 during training.
The training is continued until convergence of the parameters (typically between 100 and 300 epochs).
The sparsity parameters (see Section~\ref{sec:Training}) are set to $\mu = 0.04$, and $\phi = 0.65$, respectively.
In addition, we use a value of $0.0035$ for $L2$ weight regularization, which penalizes large weight coefficients.


\section{Results and Discussion}\label{sec:results}
We tested three different representations for pitch, yielding the following F1 scores for 10-grams: \emph{absolute pitch} (0.582), \emph{interval} (0.600), and the absolute value of interval (i.e. $|$\emph{interval}$|$) plus \emph{contour} (0.602). The latter representation was chosen for our experiments, as it showed the best performance. Not surprisingly, relative pitch representations lead to better results, as they reduce the number of combination possibilities in the input. Event though the difference in F1 score between \emph{interval} and $|$\emph{interval}$|$ \emph{plus contour} representation is not significant, it still shows that it is valid to decompose viewpoints into their elementary informative parts. Such an approach, next to reducing the input dimensionality, may also support the generalization ability of a model (e.g. $|$interval$|$ representation in music may help to understand the concept of inversion).

Figure~\ref{fig:ng_vs_f1} shows the F1 score obtained by models of different n-gram sizes.
The fact that boundary detection is reasonably good even for 1-grams is likely due to the fact that the 1-gram includes the OOI, which is mostly zero, except for the relatively rare occurrence of a rest between notes.
Because of this, the probability values assigned to OOI values by a trained RBM behave like an inverted rest indicator: high for OOI = 0, and low for OOI $>$ 0.
This makes the behaviour of the 1-gram RBM much like that of the GPR 2a rule (Section~\ref{sec:rule-based-segm}).
That GPR 2a performs slightly better (see Table~\ref{results}) can be explained by the fact that the RBM also detects segment boundaries at large (and unlikely) pitch intervals, which are not always correct.

\begin{figure}[t]
\centering\footnotesize
\includegraphics[width=0.7\linewidth]{Chapters/seg1/fig/nglen_vs_f1.pdf}
\caption{Maximal F1 scores for different n-gram lengths.}
\label{fig:ng_vs_f1}
\end{figure}

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{@{}llllc@{}}
\toprule
Model & Precision & Recall & F1 \\ \midrule
Grouper & 0.71 & 0.62 & 0.66  \\
LBDM & 0.70 & 0.60 & 0.63 \\
RBM (10-gram) & 0.83 & 0.50 & 0.60 \\
IDyOM & 0.76 & 0.50 & 0.58 \\
GPR 2a & 0.99 & 0.45 & 0.58 \\ \midrule
GPR 2b & 0.47 & 0.42 & 0.39 \\
GPR 3a & 0.29 & 0.46 & 0.35 \\
GPR 3d & 0.66 & 0.22 & 0.31 \\
PMI & 0.16 & 0.32 & 0.21 \\
TP & 0.17 & 0.19 & 0.17 \\ \midrule
Always & 0.13 & 1.00 & 0.22 \\
Never & 0.00 & 0.00 & 0.00 \\
\bottomrule
\end{tabular}
\caption{Results of the model comparison, ordered by F1 score.}
\label{results}
\end{table}

Another remarkable result is that 1-grams perform better than 2-grams (see Figure~\ref{fig:ng_vs_f1}). Although we have no definite explanation for this yet, the difference may be related to the fact that in the 1-gram model, the probability is estimated by sampling without clamping any units. In contrast, for 2-grams half the units get clamped during sampling. Prior tests with our method for computing the conditional probability (Section~\ref{sec:Posterior}) have revealed (unsurprisingly) that the quality of the approximation decreases with the ratio of unknown units over given (clamped) units. This phenomenon may also partly account for the steady increase of F1 scores for increasing n-grams sizes larger than one. Nevertheless, the increasing performance with increasing n-gram size demonstrates that the RBM based segmentation method is less susceptible to problems of data sparseness encountered in n-gram counting approaches.

\section{Conclusion}\label{sec:Conclusion and Future Work}
In this paper, an RBM-based unsupervised probabilistic method for segmentation of melodic sequences was presented.
In contrast to other statistical methods, our method does not rely on frequency counting, and thereby circumvents problems related to data sparsity.
The method performs slightly better than IDyOM, a sophisticated frequency counting model.

The segment boundary detection capabilities of our model are still slightly lower than state-of-the-art rule based methods that rely on gestalt principles formulated for musical stimuli.
This result underlines the remaining challenge to find segmentation models that correspond to human perception, based only on musical stimuli in combination with universal learning principles.

An important aspect of human perception that is missing in our current method is equivalent of short-term memory, to bias long-term expectations based on the stimuli in the direct past (see~\cite{Pearce:2010ij}).
Furthermore, we wish to investigate the effect of different architectural factors on the segmentation behaviour of the model, like an increased number of hidden layers, or an increased number of hidden units per hidden layer. 
Lastly, the formation of boundary strength profiles may be improved by involving other information theoretic quantities, such as the entropy of conditional probability distributions.

\section*{Acknowledgements}\label{sec:Acknowledgments}
The project Lrn2Cre8 acknowledges the financial support of the Future and Emerging Technologies (FET) programme within the Seventh Framework Programme for Research of the European Commission, under FET grant number 610859.
We thank Marcus Pearce for sharing the Essen data used in \cite{Pearce:2010ij}.



==> Chapters/seg2/seg2.tex <==

\chapter{Pseudo-Supervised Training Improves Unsupervised Melody Segmentation}

\begin{abstract}
An important aspect of music perception in humans is the ability to segment streams of musical events into structural units such as motifs and phrases.
A promising approach to the computational modeling of music segmentation employs the statistical and information-theoretic properties of musical data, based on the hypothesis that these properties can (at least partly) account for music segmentation in humans. Prior work has shown that in particular the information content of music events, as estimated from a generative probabilistic model of those events, is a good indicator for segment boundaries.
In this paper we demonstrate that, remarkably, a substantial increase in segmentation accuracy can be obtained by not using information content estimates directly, but rather in a bootstrapping fashion. More specifically, we use information content estimates computed from a generative model of the data as a target for a feed-forward neural network that is trained to estimate the information content directly from the data. We hypothesize that the improved segmentation accuracy of this bootstrapping approach may be evidence that the generative model provides noisy estimates of the information content, which are smoothed by the feed-forward neural network, yielding more accurate information content estimates.
\end{abstract}

\section{Introduction}\label{sec:introduction}
A prominent theory about human perception and cognition states that `chunking' is a key mechanism in human information processing~\cite{gobet01:_chunk}.
By internally representing information in `chunks'---meaningful constituents---humans are capable of interpreting information more efficiently than when information is processed in terms of lower level information units.
A prominent example of chunking has been shown in the context of chess~\cite{gobet98:_exper}, where increased skill level is associated with more efficient chunking of information about board configurations.
Moreover, chunking is involved more generally in visual~\cite{McCollough30062007} and acoustic/speech processing~\cite{baddeley66:_short} tasks.
Just as in speech, perception in terms of meaningful constituents is a principal trait of music cognition. This is immanent in the ubiquitous notion of constituent structure in music theory.

The formation of chunks involves grouping and segmentation of information. To account for those phenomena in music perception, a prominent approach from music theory and cognitive psychology has been to apply perceptual grouping mechanisms, such as those suggested by Gestalt psychology.
\emph{Gestalt principles}, such as the laws of proximity, similarity, and closure, were first discussed in visual perception \cite{wertheimer1938laws}, and have been successfully applied to auditory scene analysis \cite{bregman90} and inspired theories of music perception \cite{meyer56,narmour90,lerdahl1983generative}.
Narmour's Implication-Realization theory \cite{narmour90}, for example, uses measures of pitch proximity and closure that offer insight into how listeners perceive the boundaries between musical phrases.
This type of theory-driven approach has given rise to various rule-based computational models of segmentation.
This class of models relies upon the specification of one or more principles according to which musical sequences are grouped.

An alternative account of grouping and segmentation is based on the intuition that the distribution, or statistical structure of the sensory information, has an important effect on how we perceive constituent structure.
This idea has been explored for different areas, such as vision~\cite{glicksohn11:_gestal}, speech~\cite{Brent99anefficient}, and melody perception~\cite{pearce2010role}. The key idea is that the sensory information that comprises a chunk is relatively constant, whereas the succession of chunks (which chunk follows which) is more variable.
In information-theoretic terms, this implies that the \emph{information content} (informally: unexpectedness) of events within a chunk is lower than that of events that mark chunk boundaries.
As a side note on vocabulary: We will use the term \emph{segment}, rather than \emph{chunk} in the rest of this paper, to express that we take an agnostic stance toward the precise nature of constituents, and rather focus on their demarcation.

While Gestalt principles are sometimes rather abstractly defined laws, information theory has a certain potential to formally describe and quantify such perceptive phenomenons. The Gestalt idea of grouping based on "good form" (i.e. Pr\"agnanz), for example, has an information theoretic counterpart in the work of~\cite{von2005treatise}, where human vision is assumed to resolve ambiguous perceptive stimuli by preferring the most probable interpretation. In addition, it is intuitively clear that in most real-word scenarios, the uncertainty about expectations (i.e. the entropy) tends to increase with higher distances from observed events in any relevant dimension. Thus, while a direct link between the two paradigms is beyond dispute, the question remains which of it is more parsimonious and might have given rise for the other to emerge as a perceptual mechanism.

Prior work has shown that the information content of music events, as estimated from a generative probabilistic model of those events, is a good indicator for segment boundaries in melodies~\cite{Pearce:2010ij}.
In this paper we demonstrate that, remarkably, a substantial increase in segmentation accuracy can be obtained by not using information content estimates directly, but rather in a bootstrapping fashion.
More specifically, we use information content estimates computed from a generative model of the data as a target for a feed-forward neural network (FFNN) that is trained to estimate the information content directly from the data.

In an experimental setup, we compare our method to other methods in an evaluation against human segment boundary annotations.
Moreover, we offer an explanation for the improved accuracy by describing how our method can be regarded as employing a form of \emph{entropy regularization}~\cite{Grandvalet:2004wl}.
%\comment{is this claim accurate? } Yes, it is! 

The structure of the paper is as follows.
In Section~\ref{sec:related-work}, we discuss statistical models for melody segmentation, as well as related work regarding the pseudo-supervised regularization scheme.
In Section~\ref{sec:method}, we describe how we estimate the conditional probability and information content of notes using a Restricted Boltzmann Machine (RBM), how notes are represented as input to the model, how an FFNN is used to predict information content, and how the information content is used to predict segment boundaries.
Section~\ref{sec:Experiment} describes the experimental setup for evaluation of the model.
The results are presented and discussed in Section~\ref{sec:results-discussion}, and conclusions and future work are presented in Section~\ref{sec:concl-future-work}.


\section{Related work}\label{sec:related-work}
A notable information theory driven method for melodic segmentation is based on IDyOM, a class of variable order markov models for capturing the statistical structure of music~\cite{pearce05:_const_evaluat_statis_model_melod}.
After training on musical data, IDyOM can produce a variety of information-theoretic quantities for a given musical context, such as \emph{entropy}, expressing how confidently the model can predict the continuation of the context, and \emph{information content}, expressing how unexpected the actual continuation of the context is, under the model.
In particular the information content has been shown to be a good indicator of segment boundaries in monophonic melodies, using adaptive thresholding to predict segment boundaries when the information content (IC) of a note is high with respect to the IC values of its predecessors~\cite{Pearce:2010ij}. 

Pearce et al. compare their probabilistic melody segmentation method, along with some other information theoretic models inspired by~\cite{Brent99anefficient}, to several knowledge based methods for melody segmentation, notably \emph{Grouper}~\cite{temperley01}, \emph{LBDM}~\cite{cambouropoulos01a}, and several grouping rules that are part of the Generative Theory of Tonal Music~\cite{lerdahl1983generative}, as formalized in~\cite{Frankland:2004ug}.
The results of this comparison (that are partly reported in Section~\ref{sec:results-discussion}) show that IDyOM predicts segment boundaries much better than simpler information-theoretic methods, although not as accurately as \emph{Grouper} and \emph{LBDM}.

In prior work, we have proposed a probabilistic segmentation method analogous to IDyOM, but using an RBM as a probabilistic model of the data, rather than variable order markov models~\cite{Lattner:2015a}.
This method was shown to predict segment boundaries less accurately than \emph{Grouper} and \emph{LBDM}, but better than IDyOM.
In Sections~\ref{sec:rbm} to \ref{sec:information-content}, we recapitulate the RBM based approach to compute IC values for melody notes.
The actual contribution of this paper is an extension of this approach to what we call a \emph{pseudo-supervised} scenario (Section~\ref{sec:pseudo-superv-train}).
In this setting, rather than using the IC estimations from the RBM directly for predicting segments, they are used as targets for a FFNN, which is trained to predict IC values directly from the data (without a probabilistic model).

Although the term pseudo-supervised does not (yet) seem to have a well-established meaning, our use of the term is compatible with its use in~\cite{noklestad09:_machin_learn_approac_anaph_resol}, in the sense that a supervised approach is used to predict targets that are computed from the input data, rather than relying on hand-labeled (or otherwise authoritative) targets.
The automatically generated targets (in this case IC values) are not themselves the actual targets of interest (the boundary segments), but are instrumental to the prediction of the actual targets.

Similar methods are proposed by~\cite{Lee:2013ta} and~\cite{Hinton:2014wy}, where supervised models are used to generate targets (pseudo labels or soft-targets) from new data. But in contrast to a \emph{pseudo-supervised} approach, these methods require hand-labeled data, and are strictly taken a \emph{semi-supervised} approach, in which predictive models are trained partly in an unsupervised manner, and partly using hand-labeled data.

%\comment{todo: write a paragraph that states that in general, semi- and pseudo-suvervised approaches are beneficial because they act as a regularizer (cite entropy regularization)}
In general, both semi- and pseudo-supervised learning approaches benefit from the use of unlabeled information by using Bayesian approaches, which make assumptions over the distribution of unlabeled data. From a formal standpoint, these techniques act as regularizers of the model parameters, and thus, prevent overfitting.  Approaches like \emph{entropy regularization}~\cite{Grandvalet:2004wl} use the principle of maximum entropy to select a prior distribution of the model parameters, and then optimize the model in Maximum a Posteriori (MAP) sense.
% We propose a computational method for melody segmentation, based on a Restricted Boltzmann Machine (RBM) as a generative probabilistic model of the data. This model is used to compute the information content of each note in the melody. A first approach to melody segmentation using this model predicts segment boundaries directly from the estimated information content of notes, using an adaptive threshold. This method is analog to the one proposed in~\cite{Pearce:2010ij}, who use an dynamic n-gram model rather than an RBM for modeling the data. 

% We have found that by training a second model to predict the RBM estimates of the information content directly from the data, a substantial improvement in segmentation accuracy is achieved.

\section{Method}\label{sec:method}
In this Section, we describe the methods used to predict melody segment boundaries. We start by describing how conditional probabilities of music events can be estimated by training an RBM as a probabilistic model of the data (Section~\ref{sec:rbm}). The representation of music events is described in Section~\ref{sec:DataRepresentation}. Section~\ref{sec:information-content} details how the IC of music events is computed based on their estimated conditional probabilities. In Section~\ref{sec:pseudo-superv-train}, we describe how training a supervised model using IC values as (pseudo) targets can act as a form of regularization. Finally, Section~\ref{sec:peak-picking} describes how segment boundaries are predicted from sequences of IC values.

\subsection{Probability approximation through Monte Carlo techniques} \label{sec:rbm}
An RBM is a stochastic Neural Network with two layers, a visible layer with units $\mathbf{v} \in \{0,1\}^r$ and a hidden layer with units $\mathbf{h} \in \{0,1\}^q$ \cite{Hinton:2002ic}.
The units of both layers are fully interconnected with weights $\mathbf{W} \in \mathbb{R}^{r \times q}$, while there are no connections between the units within a layer.

In a trained RBM, the marginal probability distribution of a visible configuration $\mathbf{v}$ is given by the equation
\begin{equation}
p(\mathbf{v}) = \frac{1}{Z} \sum_{\mathbf{h}}{e^{-E(\mathbf{v}, \mathbf{h})}},
\end{equation}
where $E(\mathbf{v}, \mathbf{h})$ is an energy function.
The computation of this probability distribution is intractable, because it requires summing over all possible joint configurations of $\mathbf{v}$ and $\mathbf{h}$ as
\begin{equation}
Z = \sum_{\mathbf{v},\mathbf{h}}{e^{-E(\mathbf{v},\mathbf{h})}}.
\end{equation}

However, with Monte Carlo techniques it is possible to approximate the probability of a visible unit configuration $\mathbf{v}$. To that end, for $N$ randomly initialized \emph{fantasy particles}\footnote{See \cite{tielemanPcd2008}} $\mathbf{Q}$, we execute Gibbs sampling until thermal equilibrium. In the visible \emph{activation vector} $\mathbf{q}_i$ of a fantasy particle $i$, element $q_{ij}$ specifies the probability that visible unit $j$ is on. Since all visible units are independent given $\mathbf{h}$, a single estimate based on one fantasy particles visible activation is computed as

\begin{equation}
p(\mathbf{v} | \mathbf{q}_i) = \prod_j{p(v_j | q_{ij})}.
\end{equation}

As we are using binary units, such an estimate can be calculated by using a binomial distribution with one trial per unit.
We average the results over $N$ fantasy particles, leading to an increasingly close approximation of the true probability of $\mathbf{v}$ as N increases:

\begin{equation}\label{binomial}
p(\mathbf{v} | \mathbf{Q}) = \frac{1}{N}\sum_i^N{\prod_j{\binom{1}{v_j}q_{ij}^{v_j}(1-q_{ij})^{1-v_j}}}.
\end{equation}

\subsubsection{Posterior probabilities of visible units}\label{sec:Posterior}
When the visible layer consists of many units, $N$ will need to be very large to obtain good probability estimates with the method described above.
However, for conditioning a small subset of visible units $\mathbf{v}_s \subset \mathbf{v}$ on the remaining visible units $\mathbf{v}_c = \mathbf{v} \setminus \mathbf{v}_s$, the above method is very useful.
This can be done by Gibbs sampling after randomly initializing the units $\mathbf{v}_s$ while clamping all other units $\mathbf{v}_c$ according to their initial state in $\mathbf{v}$.
In Eq.
\ref{binomial}, all $\mathbf{v}_c$ contribute a probability of $1$, which results in the conditional probability of $\mathbf{v}_s$ given $\mathbf{v}_c$.

We use this approach to condition the units belonging to the last time step of an n-gram on the units belonging to preceding time steps. For the experiments reported in this paper, we found that it is sufficient to use 150 fantasy particles and for each to perform 150 Gibbs sampling steps.

\subsubsection{Training}\label{sec:Training}

We train a single RBM using \emph{persistent contrastive divergence} (PCD)~\cite{tielemanPcd2008} with \emph{fast weights}~\cite{tielemanFpcd2009}, a variation of the standard \emph{contrastive divergence} algorithm~\cite{hinton06}.
This method yields models which are well-suited for sampling, because it results in a better approximation of the likelihood gradient.

Based on properties of neural coding, sparsity and selectivity can be used as constraints for the optimization of the training algorithm~\cite{Goh:2010wi}.
Sparsity encourages competition between hidden units, and selectivity prevents over-dominance by any individual unit.
A parameter $\mu$ specifies the desired degree of sparsity and selectivity, whereas another parameter $\phi$ determines how strongly the sparsity/selectivity constraints are enforced. 

\subsection{Data Representation}\label{sec:DataRepresentation}

From the monophonic melodies, we construct a set of n-grams by using a sliding window of size n and a step size of 1.
For each note in the n-gram, four basic features are computed: 1) absolute values of the pitch interval between the note and its predecessor (in semitones); 2) the contour (up, down, or equal); 3) inter-onset-interval; and 4) onset-to-offset-interval. The IOI and OOI values are quantized into semiquaver and quaver, respectively.
Each of these four features is represented as a binary vector and its respective value for any note is encoded in a one-hot representation. The first n-1 n-grams in a melody are noise-padded to account for the first n-1 prefixes of the melody. Some examples of binary representations of n-grams are given in Figure~\ref{fig:Representation}).

\begin{figure}[t]
\centering\footnotesize
\includegraphics[width=\linewidth]{Chapters/seg2/fig/ngrams.pdf}
\caption{Seven examples of n-gram training instances (n=10) used as input to the RBM.
Within each instance (delimited by a dark gray border), each of the 10 columns represents a note.
Each column consists of four \emph{one-hot} encoded viewpoints: $|$\emph{interval}$|$, \emph{contour}, \emph{IOI} and \emph{OOI} (indicated by the braces on the left). The viewpoints are separated by horizontal light gray lines for clarity.
The first instance shows an example of noise padding (in the first six columns) to indicate the beginning of a melody.}
\label{fig:Representation}
\end{figure}

\subsection{Information Content}\label{sec:information-content}

After we trained the model as described in Section \ref{sec:Training}, we estimate the probability of the last note conditioned on its preceding notes for each n-gram as introduced in Section \ref{sec:Posterior}.
From the probabilities $p(e_t \mid e_{t-n+1}^{t-1})$ computed in this way, we calculate the IC as

\begin{equation}\label{eq:ic}
h(e_t \mid e_{t-n+1}^{t-1}) = log_2 \frac{1}{p(e_t \mid e_{t-n+1}^{t-1})},
\end{equation}
where $e_t$ is a note event at time step t, and $e_k^l$ is a note sequence from position $k$ to $l$ of a melody.
IC is a measure of the unexpectedness of an event given its context.
According to a hypothesis of~\cite{Pearce:2010ij}, segmentation in auditory perception is determined by perceptual expectations for auditory events.
In this sense, the IC relates directly to this perceived boundary strength, thus we refer to the IC over a note sequence as the \emph{boundary strength profile} (BSP).


\subsection{Pseudo-Supervised optimization}\label{sec:pseudo-superv-train}

\begin{algorithm}
\KwData{ Set of n-grams : $\mathbf{V}=\{ \mathbf{v}_1, \dots, \mathbf{v}_N\}$}
Train an RBM by optimizing the model parameters as
\begin{equation}
\tilde \theta = \argmax_\theta \log p(\mathbf{v} \mid \theta)
\label{eq:rbm_pretrain}
\end{equation}
 
 Compute the set of \emph{pseudo-targets} $\mathbf{T}=\{\mathbf{t}_1,\dots,\mathbf{t}_N\}$ as 
  \begin{align}
 \mathbf{t}_t(\mathbf{v}_t ; \tilde \theta) = h(e_t \mid e_{t-n+1}^{t-1}), 
 \end{align}
 where $\mathbf{v}_t$ is the encoding of the n-gram $\{e_{t-n+1}, \dots, e_{t}\} $, and $h(e_t \mid e_{t-n+1}^{t-1})$ is the IC computed as in Eq.~\eqref{eq:ic}.

Build a three layered FFNN and optimize it in a supervised way, using the set of pseudo-targets $\mathbf{T}$ as
 \begin{equation}
 \hat \theta = \argmin_\theta \sum_{i=1}^N\norm{\mathbf{t} (\mathbf{v}_t; \tilde \theta)- \mathbf{y}(\mathbf{v}_t ; \theta)}^2,
 \label{eq:ffnn_train}
 \end{equation}
 where $\mathbf{y}(\mathbf{v}_t; \theta)$ is the output of the FFNN for $\mathbf{v}_t$ given the model parameters $\theta$.
 
 \Return 
Model parameters $\hat \theta$
 \caption{Pseudo-supervised training} \label{alg:pseudo_supervised}
 \label{algo}
\end{algorithm}

In contrast to our prior work, we do not use the BSP estimated from the RBM for segmentation. Instead, we train an FFNN to predict the estimated BSP directly from the data in a non-probabilistic manner, and use that curve for predicting segment boundaries (by the procedure described in Section~\ref{sec:peak-picking}). This is a way of context sensitive smoothing, which is achieved by the generalization ability of the NN. Note that no labeled data is used at any stage of the processing pipeline. The fact that this approach still improves the segmentation results is evidence that the generative model, as described in Section \ref{sec:rbm}, provides noisy IC estimates. This is either due to poor approximations to the actual IC by the model itself, or the data can be considered to be noisy with respect to prototypical segment endings.

The proposed pseudo-supervised training method is shown in Algorithm~\ref{alg:pseudo_supervised}. Formally, this method is an approximate MAP estimation of the parameters using entropy regularization \cite{Grandvalet:2004wl}. In this method, the MAP estimate of the model parameters is computed as
\begin{equation}
\theta_{MAP} =  \argmax_\theta \log p(\mathbf{v} \mid \theta) - \lambda  H(\mathbf{t} \mid \mathbf{v} ; \theta),
\label{eq:map}
\end{equation}
where $H(\mathbf{t} \mid \mathbf{v})$ is the conditional Shannon entropy of the targets  given the inputs, and $\lambda$ is a Lagrange multiplier. In the proposed algorithm, this approximation is obtained by independently optimizing $\log p(\mathbf{v} \mid \theta)$ (see Eq.~\eqref{eq:rbm_pretrain}), and then minimizing Eq.~\eqref{eq:ffnn_train}, which is equivalent to maximizing 
\begin{equation}
p(\mathbf{t} \mid \mathbf{v}; \theta,\beta) = \mathcal{N} (\mathbf{t} \mid \mathbf{y}(\mathbf{v}, \theta), \beta^{-1}),
\end{equation}
where $\beta$ is the precision (inverse variance) of the distribution. This precision can be found by minimizing the negative log-likelihood of the above probability to give
\begin{equation}
\beta = \frac{N}{\sum_{i} \norm{\mathbf{t}_i - \mathbf{y}(\mathbf{v}_i, \theta)}^2}.
\end{equation}
The Shannon entropy for this distribution is given by
\begin{align}
H(\mathbf{t} \mid \mathbf{v} ; \theta, \beta) &=  \mathbb{E} \left\{ -  \log p(\mathbf{t} \mid \mathbf{v}) \right\} \notag \\
&= \frac{1}{2} \log \left( \frac{2\pi}{\beta}\right) + \frac{1}{2},
\end{align}
 which is minimal, since $\sum_{i} \norm{\mathbf{t}_i - \mathbf{y}(\mathbf{v}_i, \theta)}^2$ is minimal. Therefore, optimizing Eq.~\eqref{eq:ffnn_train} is equivalent to minimizing the entropy term in Eq.~\eqref{eq:map}.

 We use the fact that the RBM is a generative model, and therefore, the pseudo targets $\mathbf{t}$ come from the computation of the IC from a probabilistically sound estimate of the input data. In this way, pseudo-supervised learning can be understood as a suboptimal entropy-regularized MAP model of the model parameters.

\subsubsection{Training}
To compute $\hat{\theta}$ in Equation~(\ref{eq:ffnn_train}), we use a three layered FFNN with sigmoid hidden units and a single linear unit in the output layer. We pre-train the hidden layer with PCD and fine-tune the whole stack with Backpropagation, by minimizing the mean square error. As targets, we use the boundary strength values, estimated by the initial model described in Section \ref{sec:Posterior}.

After training, the outputs $\mathbf{y}(\mathbf{v}_i ; \hat{\theta})$ of the FFNN are used as (improved) estimates of the information content of $e_t$, given $\{e_{i-n+1}, \dots, e_{t-1}\}$.

\subsection{Peak Picking}\label{sec:peak-picking}
Based on the BSP described in Section \ref{sec:information-content} and the outputs $\mathbf{y}(\mathbf{v}_i ; \hat{\theta})$ of the FFNN (see Algorithm \ref{algo}), respectively, we need to find a discrete binary segmentation vector.
For that, we use the peak picking method described in~\cite{Pearce:2010ij}.
This method finds all peaks in the profile and keeps those which are $k$ times the standard deviation greater than the mean boundary strength, linearly weighted from the beginning of the melody to the preceding value:

\begin{equation}
S_n > k \sqrt{\frac{\sum_{i=1}^{n-1}{(w_i S_i - \bar{S}_{w,1\dots n-1})^2}}{\sum_1^{n-1}{w_i}}} + \frac{\sum_{i=1}^{n-1}{w_i S_i}}{\sum_1^{n-1}{w_i}},
\end{equation}
where $S_m$ is the $m$-th value of the BSP, and $w_i$ are the weights which emphasize recent values over those of the beginning of the song (triangular window), and $k$ has to be found empirically.

\section{Experiment}\label{sec:Experiment}
To allow for a comparison of our segmentation method with other approaches, the experimental setup of the proposed method follows~\cite{Pearce:2010ij} both in terms of data and procedure.

\subsection{Data}\label{sec:TrainingData}
%The Essen Folk Song Collection (EFSC) \comment{[Helmut Schaffrath]} is a widely used corpus for MIR experiments on symbolic music.

For training and testing, we use the Essen Folk Song Collection (EFSC)~\cite{TheEssenFolksongC:1995um}, a widely used corpus in music information retrieval (MIR). This database   consists of more than 6000 transcriptions of folksongs primarily from Germany and other European regions.
Due to the fact that phrase markers are encoded, the EFSC is one of the most used collections for testing computational models of music segmentation.

In accordance with~\cite{Pearce:2010ij}, we use the \emph{Erk} subset of the EFSC, which consists of 1705 German folk melodies with a total of $78,995$ note events.
Encoded phrase boundary annotations in the corpus constitute the baseline of about $12\%$ positive examples.

\subsection{Procedure}

The model is trained and tested on the data described in Section~\ref{sec:TrainingData} with various n-gram lengths between 3 and 10. For each n-gram length, we perform 5-fold cross-validation and average the results over all folds.
Similar to the approach in~\cite{Pearce:2010ij}, after computing the BSPs, we evaluate different $k$ from the set $\{0.70, 0.75, 0.80, 0.85, 0.90, 0.95, 1.00\}$ (initial IC estimation), and $\{0.24, 0.26, 0.28, 0.30, 0.32, 0.34, 0.36\}$ (after pseudo-supervised optimization), and choose the value that maximizes F1 for the respective n-gram length.
To make results comparable to those reported in~\cite{Pearce:2010ij}, the output of the model is appended with an implicit (and correct) phrase boundary at the end of each melody.

Since the hyper-parameters of the model are inter-dependent, it is infeasible to exhaustively search for the optimal parameter setting.
We have manually chosen a set of hyper-parameters that give reasonable results for the different models tested. For the initial IC estimation, we use 200 hidden units, a momentum of 0.6, and a learning rate of 0.0085 which we linearly decrease to zero during training. With increasing n-gram length we linearly adapt the batch size from 250 to 1000. In addition, we use $50\%$ dropout on the hidden layer and 20\% dropout on the visible layer.

The fast weights used in the training algorithm (see Section~\ref{sec:Training}) help the fantasy particles mix well, even with small learning rates.
The learning rate of the fast weights is increased from 0.002 to 0.007 during training.
The training is continued until convergence of the parameters (typically between 100 and 300 epochs).
The sparsity parameters (see Section~\ref{sec:Training}) are set to $\mu = 0.04$, and $\phi = 0.65$, respectively.
In addition, we use a value of $0.0035$ for $L2$ weight regularization, which penalizes large weight coefficients.

For pre-training of the first layer in the FFNN, we change the learning rate to 0.005, leave the batch size constant at 250 and increase the weight regularization to 0.01. We again use dropout, for both the pre-training and the fine-tuning. 
%In fact, dropout has a major influence on the quality of the results (see \ref{fig:curves} \comment{Dangling ref}).

\section{Results and discussion}\label{sec:results-discussion}

\begin{figure}[t]
\centering\footnotesize
\includegraphics[width=\linewidth]{Chapters/seg2/fig/nglen_vs_f1.pdf}
\caption{F1 scores for different N-gram lengths and methods.}
\label{fig:f_scores}
\end{figure}

Figure \ref{fig:f_scores} shows the F1 scores for different N-gram lengths and methods. By using dropout, the F1 score increases considerably, as dropout improves the generalization abilities of the RBM. With the pseudo-supervised approach, again a significant improvement of the classification accuracy can be achieved. This is remarkable, considering that no additional information was given to the FFNN, the improvement was based solely on context-sensitive smoothing.

Figure \ref{fig:trends} shows the adaptation of single IC values through the pseudo-supervised optimization. Some previously true positives are erroneously regularized downwards (green lines from upper left to lower right), while some previously false negatives are correctly moved upwards (green lines from lower left to upper right). Quantitative tests show that our method increases IC values at boundaries more often than it decreases them. In general, if the initial BSP curve is correct in most cases, in pseudo-supervised training such regularities are detected and utilized.

Table~\ref{results} shows prediction accuracies in terms of precision, recall, and F1 score, both for our method and for the various alternative approaches mentioned in Section~\ref{sec:related-work}. The table shows that with the proposed method (RBM10+DO+PS), an information-theoretic approach is now on a par with a Gestalt-based approach (LBDM), while Grouper still provides the best estimates of melodic segment boundaries. However, Grouper exploits additional domain knowledge like musical parallelism, whereas the LBDM model, as well as (RBM10+DO+PS), are pure representatives of the Gestalt-based paradigm and the information-theoretic paradigm, respectively.

The \emph{GPR 2a} method is a simple rule that predicts a boundary whenever a rest occurs between two successive notes. Note how \emph{GPR 2a} accounts for a large portion of the segment boundaries (approx. 45\%). This implies that the challenge is mainly in recognizing boundaries that do not co-occur with a rest. For boundaries without rests, the pseudo-supervised approach yields an improvement of $3.7\%$ in the F-score, while boundaries indicated by a rest did not improve any more (as for those boundaries the initial approach already yields an F-score of $0.99$).

%\begin{figure*}
%    \centering
%    \begin{subfigure}[b]{0.5\textwidth}
%        \centering
%        \includegraphics[height=2.5in]{fig/hist_initial.pdf}
%    \end{subfigure}%
%    ~ 
%    \begin{subfigure}[b]{0.5\textwidth}
%        \centering
%        \includegraphics[height=2.5in]{fig/hist_pseudo.pdf}
%    \end{subfigure}
%    \caption{Histogram of IC curve values computed from 10-grams, grouped by ground truth labels (pos / neg). \emph{Left:} Distribution of initial IC estimation. \emph{Right:} Distribution after pseudo-supervised training.}
%\end{figure*}

\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{Chapters/seg2/fig/ic-change.pdf}
   \caption{The effect of pseudo-training on estimated IC values; Line segments connect IC values estimated directly from the probabilistic model (RBM10+DO) with the corresponding IC values after pseudo-training (RBM10+DO+PS); Green lines indicate music events that mark a segment boundary, red lines indicate those that do not.}
   \label{fig:trends}
\end{figure}

\begin{table}[t]
\centering
\begin{tabular}{@{}llllc@{}}
\toprule
Model & Precision & Recall & F1 \\ \midrule
Grouper & 0.71 & 0.62 & 0.66  \\
LBDM & 0.70 & 0.60 & 0.63 \\
\textbf{RBM10+DO+PS} & \textbf{0.80} & \textbf{0.55} & \textbf{0.63} \\
RBM10+DO & 0.78 & 0.53 & 0.61 \\
RBM10 & 0.83 & 0.50 & 0.60 \\
IDyOM & 0.76 & 0.50 & 0.58 \\
GPR 2a & 0.99 & 0.45 & 0.58 \\ % \midrule
% GPR 2b & 0.47 & 0.42 & 0.39 \\
% GPR 3a & 0.29 & 0.46 & 0.35 \\
% GPR 3d & 0.66 & 0.22 & 0.31 \\
% PMI & 0.16 & 0.32 & 0.21 \\
% TP & 0.17 & 0.19 & 0.17 \\ \midrule
% Always & 0.13 & 1.00 & 0.22 \\
% Never & 0.00 & 0.00 & 0.00 \\
\bottomrule
\end{tabular}
\caption{Results of the model comparison, ordered by F1 score. RBM results are shown for 10-grams of the initial RBM, the RBM with Dropout (DO) and the RBM with Pseudo-Supervised training (PS).
Table adapted from \protect \cite{Pearce:2010ij}, with permission.}
\label{results}
\end{table}


%\comment{Add plot of curves (initial, pseudo) and piano roll.}


\section{Conclusion and future work}\label{sec:concl-future-work}
In this paper, we show how a technique we call \emph{pseudo-supervised} training improves the prediction accuracy of a probabilistic method for melody segmentation. Our method is a purely probabilistic method, that does not rely on any knowledge about musical structure. We use the information content (IC) of musical events (estimated from a probabilistic model) as a proxy for the actual target to be predicted (segment boundaries). With these \emph{pseudo targets}, we train a feed-forward neural network. We show that segment boundaries estimated from the output of this network are more accurate than boundaries estimated from the \emph{pseudo targets} themselves.

In this paper, we used the IC as estimated from an RBM, but the pseudo-supervised approach may benefit from including IC estimates from other models, such as IDyOM~\cite{pearce05:_const_evaluat_statis_model_melod}. In addition, there are other probabilistic architectures, such as conditional RBMs~\cite{Taylor:2006vl}, that seem appropriate for estimating IC values from data. Furthermore, although the focus of this paper has been on IC, it is intuitively clear that IC is not the only factor that determines the perception of segment boundaries in melodies. Future experimentation is necessary to determine whether (combinations of) other information-theoretic quantities are also helpful in detecting melodic segment boundaries. Finally, we wish to investigate whether there are further problems where our method could be beneficial. In general, pseudo-supervised optimization could improve features which are noisy either because of the way they are calculated, or because of noise in the data on which the features are based on.

\section*{Acknowledgments}
The project Lrn2Cre8 acknowledges the financial support of the Future and Emerging Technologies (FET) programme within the Seventh Framework Programme for Research of the European Commission, under FET grant number 610859.
We thank Marcus Pearce for sharing the Essen data used in \cite{Pearce:2010ij}.

\clearpage

